Replacement Learning: Training Neural Networks with Fewer Parameters

End-to-end training with full-depth backpropagation remains the dominant paradigm for optimizing deep neural networks, but its efficiency deteriorates as models grow deeper. Since every block must be executed and differentiated under a single global objective, full-depth BP introduces substantial parameter redundancy, activation-memory cost, and training latency, especially when neighboring layers exhibit highly correlated learning patterns. Directly skipping or removing layers can reduce cost, but often weakens representation capacity or requires architecture-specific reuse designs. In this paper, we propose Replacement Learning (RepL), a training-time paradigm that reduces full-depth redundancy by replacing selected blocks rather than simply discarding them. For each removed block, RepL inserts a lightweight computing layer that synthesizes a surrogate operator from the parameters of its adjacent preceding and succeeding blocks through a learnable transformation, and applies the synthesized operator to the preceding activation. In this way, RepL preserves local contextual continuity while avoiding unnecessary full-layer computation. We instantiate RepL for CNNs and ViTs with tailored parameter-fusion blocks that handle convolutional channels, feature resolutions, and transformer submodules. Extensive experiments on CIFAR-10, SVHN, STL-10, ImageNet, COCO, and CityScapes show that RepL reduces trainable parameters, GPU memory usage, and training time while matching or surpassing standard end-to-end training across classification, detection, and segmentation. Additional results on WikiText-2, transfer learning, inference throughput, checkpointing, stochastic depth, and INT8 quantization further demonstrate its generality and compatibility.

==> sections/exp_ori.tex <==
\section{Experiments}
\subsection{Experimental setup}
We conduct classification and detection experiments using different architectures on five benchmark datasets: CIFAR-10 \cite{r1}, STL-10 \cite{r3}, SVHN \cite{r2}, ImageNet \cite{r4}, and COCO \cite{r51}. All models are trained from scratch without using any pre-trained weights. We set $k=4$ as the interval for the removed layer, and all layers compute the loss using gradient descent and update parameters via backpropagation \cite{r12}.

For the small-scale datasets (CIFAR-10, SVHN, and STL-10), we employ ViT-Tiny/8 \cite{r14}, ResNet-32, and ResNet-110 \cite{r5}, with training performed on a single Nvidia A100 GPU. For the ViT models, we use a batch size of 512 and the AdamW optimizer with a learning rate of 1e-3, training for 250 epochs. For the ResNet models, we use a batch size of 1024 and the SGD optimizer with a learning rate of 0.8, also training for 250 epochs. The data augmentation strategies are as follows: on CIFAR-10, 4-pixel reflection padding followed by random cropping back to 32$\times$32 and horizontal flipping with probability 0.5; on SVHN, random cropping to 32$\times$32 (with 2-pixel padding) without horizontal flipping; on STL-10, random cropping to 96$\times$96 (with 4-pixel padding) and horizontal flipping with probability 0.5.

For ImageNet, we conduct experiments on 4 Nvidia A100 GPUs. ViT-Tiny/16 and ViT-Small/16 are trained with a batch size of 1024 and the AdamW optimizer at a learning rate of 7.5e-4, while ResNet-34, ResNet-101, and ResNet-152 are trained with a batch size of 512 and the SGD optimizer at a learning rate of 0.2, for 90 epochs. During training, we apply a 224$\times$224 random crop with random horizontal flipping; at test time, images are resized and then center-cropped to 224$\times$224.

\subsection{Comparison with the End-to-End(E2E) results}
\subsubsection{\textbf{Results on CIFAR-10, SVHN, and STL-10}}

\begin{table*}[t]
\caption{Performance of different backbones on various datasets. RepL represents Replacement Learning. }
\label{t1}
\centering
\scalebox{1.0}{%
\setlength{\tabcolsep}{5pt}
\setlength{\tabcolsep}{5.0mm}
\begin{tabular}{cccccc}
\toprule
\textbf{Dataset} & \textbf{Backbone} & \textbf{Method} &
\textbf{Test Accuracy (\%)} & \textbf{GPU Memory (GB)} &
\textbf{Training Time (s/epoch)} \\ \midrule

\multirow{7}{*}{CIFAR-10}
& \multirow{2}{*}{ResNet-32} & E2E
& 93.17$\pm$0.14 & 3.38 & 10.44 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}93.43$\pm$0.19 ($\uparrow$0.26)
& \cellcolor[HTML]{E6F0FF}2.69 ($\downarrow$20.4\%)
& \cellcolor[HTML]{E6F0FF}8.20 ($\downarrow$21.5\%) \\ \cline{2-6}
%
& \multirow{2}{*}{ResNet-110} & E2E
& 93.49$\pm$0.29 & 9.31 & 26.19 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}94.01$\pm$0.17 ($\uparrow$0.52)
& \cellcolor[HTML]{E6F0FF}7.62 ($\downarrow$18.2\%)
& \cellcolor[HTML]{E6F0FF}20.93 ($\downarrow$20.1\%) \\ \cline{2-6}
%
& \multirow{3}{*}{ViT-Tiny/8} & E2E
& 72.77$\pm$1.31 & 2.81 & 6.81 \\
&                               & Skip-Attention
& 72.60$\pm$3.57($\downarrow$0.17) & 2.12($\downarrow$24.6\%) & 6.23($\downarrow$8.5\%) \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}73.71$\pm$1.08 ($\uparrow$0.94)
& \cellcolor[HTML]{E6F0FF}2.08 ($\downarrow$26.0\%)
& \cellcolor[HTML]{E6F0FF}5.65 ($\downarrow$17.0\%) \\ \midrule

\multirow{7}{*}{SVHN}
& \multirow{2}{*}{ResNet-32} & E2E
& 96.83$\pm$0.15 & 3.38 & 13.89 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}96.97$\pm$0.12 ($\uparrow$0.14)
& \cellcolor[HTML]{E6F0FF}2.69 ($\downarrow$20.4\%)
& \cellcolor[HTML]{E6F0FF}11.94 ($\downarrow$14.0\%) \\ \cline{2-6}
%
& \multirow{2}{*}{ResNet-110} & E2E
& 96.93$\pm$0.24 & 9.31 & 37.38 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}97.06$\pm$0.27 ($\uparrow$0.13)
& \cellcolor[HTML]{E6F0FF}7.62 ($\downarrow$18.2\%)
& \cellcolor[HTML]{E6F0FF}30.08 ($\downarrow$19.5\%) \\ \cline{2-6}
%
& \multirow{3}{*}{ViT-Tiny/8} & E2E
& 85.99$\pm$0.71 & 2.81 & 10.07 \\
&                               & Skip-Attention
& 86.22$\pm$1.51($\uparrow$0.23) & 2.12($\downarrow$24.6\%) & 9.18($\downarrow$8.8\%) \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}86.67$\pm$1.18 ($\uparrow$0.68)
& \cellcolor[HTML]{E6F0FF}2.08 ($\downarrow$26.0\%)
& \cellcolor[HTML]{E6F0FF}8.08 ($\downarrow$19.8\%) \\ \midrule

\multirow{7}{*}{STL-10}
& \multirow{2}{*}{ResNet-32} & E2E
& 79.81$\pm$0.51 & 3.38 & 5.11 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}80.33$\pm$0.42 ($\uparrow$0.52)
& \cellcolor[HTML]{E6F0FF}2.69 ($\downarrow$20.4\%)
& \cellcolor[HTML]{E6F0FF}4.13 ($\downarrow$19.2\%) \\ \cline{2-6}
%
& \multirow{2}{*}{ResNet-110} & E2E
& 79.78$\pm$0.30 & 9.31 & 6.86 \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}80.45$\pm$0.51 ($\uparrow$0.67)
& \cellcolor[HTML]{E6F0FF}7.62 ($\downarrow$18.2\%)
& \cellcolor[HTML]{E6F0FF}5.23 ($\downarrow$23.8\%) \\ \cline{2-6}
%
& \multirow{3}{*}{ViT-Tiny/8} & E2E
& 49.08$\pm$3.39 & 2.81 & 2.93 \\
&                               & Skip-Attention
& 50.42$\pm$3.18($\uparrow$1.34) & 2.12($\downarrow$24.6\%) & 2.68($\downarrow$8.5\%) \\
&                               & \cellcolor[HTML]{E6F0FF}RepL
& \cellcolor[HTML]{E6F0FF}50.66$\pm$3.18 ($\uparrow$1.58)
& \cellcolor[HTML]{E6F0FF}2.08 ($\downarrow$26.0\%)
& \cellcolor[HTML]{E6F0FF}2.41 ($\downarrow$17.8\%) \\
\bottomrule
\end{tabular}}
\end{table*}
% We evaluate our method on CIFAR-10 \cite{r1}, SVHN \cite{r2}, and STL-10 \cite{r3}, with results in Table \ref{t1}. 
\tyh{We evaluate our method on CIFAR-10 \cite{r1}, SVHN \cite{r2}, and STL-10 \cite{r3} and present the results in Table \ref{t1}. }
The results reveal that Replacement Learning (RepL) consistently outperforms E2E training \cite{r12} across all architectures: On CIFAR-10 \cite{r1}, ResNet-32/110 \cite{r5} test accuracy rises from 93.17 to 93.43 and 93.49 to 94.01, while ViT-Tiny/8 \cite{r14} gains 0.94; on SVHN \cite{r2}, accuracy increases by 0.13 at least across networks; on STL-10 \cite{r3}, gains range from 0.52 to 1.58, with consistent significant improvements across datasets. Table \ref{t1} also shows RL’s advantages on CIFAR-10 \cite{r1}: ResNet-32/110 \cite{r5}, and ViT-Tiny/8 \cite{r14} reduce GPU memory by 0.69/1.69/0.73 GB, and training time per epoch by 21.5\%, 20.1\%, 17.0\% respectively. Similar trends hold for SVHN \cite{r2} and STL-10 \cite{r3}, where RL cuts memory and training time while maintaining or improving performance.

Furthermore, when compared to Skip-Attention \cite{r21} on ViTs \cite{r14}, our method outperforms both in terms of performance and resource efficiency, making it a more favorable choice for maintaining accuracy while reducing computational cost.
\subsubsection{\textbf{Results on ImageNet}}
\begin{table*}[t]
\caption{Results on the ImageNet validation set. RepL stands for Replacement Learning.}
\label{t2}
\centering
\scalebox{1.0}{%
\setlength{\tabcolsep}{5pt}
\setlength{\tabcolsep}{5.4mm}
\begin{tabular}{cccccc}
\toprule
\textbf{Backbone} & \textbf{Method} &
\textbf{\begin{tabular}[c]{@{}c@{}}Top-1\\Accuracy (\%)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Top-5\\Accuracy (\%)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}GPU Memory\\(GB)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Training Time\\(s/epoch)\end{tabular}} \\ \midrule
\multirow{2}{*}{ResNet-34}
& E2E & 74.82$\pm$1.43 & 91.04$\pm$1.33 & 9.21 & 463.23 \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}75.44$\pm$1.27 ($\uparrow$0.62)
  & \cellcolor[HTML]{E6F0FF}91.47$\pm$2.01 ($\uparrow$0.43)
  & \cellcolor[HTML]{E6F0FF}8.06 ( $\downarrow$12.5\% )
  & \cellcolor[HTML]{E6F0FF}410.53 ( $\downarrow$11.4\% ) \\ \cline{1-6}
\multirow{2}{*}{ResNet-101}
& E2E & 77.55$\pm$1.22 & 93.80$\pm$1.78 & 20.95 & 720.11 \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}78.13$\pm$1.65 ($\uparrow$0.58)
  & \cellcolor[HTML]{E6F0FF}94.02$\pm$1.34 ($\uparrow$0.22)
  & \cellcolor[HTML]{E6F0FF}18.05 ( $\downarrow$13.8\% )
  & \cellcolor[HTML]{E6F0FF}616.23 ( $\downarrow$14.4\% ) \\ \cline{1-6}
\multirow{2}{*}{ResNet-152}
& E2E & 78.16$\pm$1.56 & 94.03$\pm$1.25 & 27.58 & 738.74 \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}78.31$\pm$1.46 ($\uparrow$0.15)
  & \cellcolor[HTML]{E6F0FF}94.14$\pm$1.14 ($\uparrow$0.11)
  & \cellcolor[HTML]{E6F0FF}24.19 ( $\downarrow$12.3\% )
  & \cellcolor[HTML]{E6F0FF}633.89 ( $\downarrow$14.2\% ) \\ \cline{1-6}
\multirow{3}{*}{ViT-T/16}
& E2E & 60.23$\pm$1.52 & 82.38$\pm$1.32 & 12.17 & 357.66 \\
& Skip-Attn
  & 60.51$\pm$1.20($\uparrow$0.28) & 82.72$\pm$1.09($\uparrow$0.34)
  & 11.52 ( $\downarrow$5.3\% )
  & 381.44 ( $\uparrow$6.7\% ) \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}60.93$\pm$1.19 ($\uparrow$0.70)
  & \cellcolor[HTML]{E6F0FF}82.88$\pm$1.07 ($\uparrow$0.50)
  & \cellcolor[HTML]{E6F0FF}9.59 ( $\downarrow$21.2\% )
  & \cellcolor[HTML]{E6F0FF}290.15 ( $\downarrow$18.9\% ) \\ \cline{1-6}
\multirow{3}{*}{ViT-S/16}
& E2E & 64.35$\pm$1.83 & 84.64$\pm$1.22 & 21.05 & 798.61 \\
& Skip-Attn
  & 61.65$\pm$1.25($\downarrow$2.70) & 82.70$\pm$1.16($\downarrow$1.94)
  & 20.67 ( $\downarrow$1.8\% )
  & 755.14 ( $\downarrow$5.4\% ) \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}65.09$\pm$1.41 ($\uparrow$0.74)
  & \cellcolor[HTML]{E6F0FF}85.42$\pm$1.73 ($\uparrow$0.78)
  & \cellcolor[HTML]{E6F0FF}16.22 ( $\downarrow$22.9\% )
  & \cellcolor[HTML]{E6F0FF}617.10 ( $\downarrow$22.7\% ) \\
\midrule
\multirow{3}{*}{ViT-B/16}
& E2E & 59.46$\pm$1.72 & 80.35$\pm$1.12 & 41.97 & 2566.70 \\
& Skip-Attn
  & 58.94$\pm$1.25($\downarrow$0.52) & 79.70$\pm$0.94($\downarrow$0.65)
  & 38.49 ( $\downarrow$8.3\% )
  & 2393.81 ( $\downarrow$6.7\% ) \\
& \cellcolor[HTML]{E6F0FF}RepL
  & \cellcolor[HTML]{E6F0FF}60.18$\pm$1.27 ($\uparrow$0.72)
  & \cellcolor[HTML]{E6F0FF}81.97$\pm$1.15 ($\uparrow$1.62)
  & \cellcolor[HTML]{E6F0FF}29.94 ( $\downarrow$28.7\% )
  & \cellcolor[HTML]{E6F0FF}1924.35 ( $\downarrow$25.1\% ) \\
\bottomrule
\end{tabular}}
\end{table*}
We systematically validate RepL’s effectiveness on ImageNet \cite{r4} with ResNet-34/101/152 \cite{r5}, and ViT-Tiny/16, ViT-Small/16, and ViT-Base/16 \cite{r14}, with comprehensive experimental results summarized in \cref{t2}. For ResNet-34 \cite{r5} as a representative case, Top-1 Accuracy rises from 74.82 to 75.44, and Top-5 Accuracy increases from 91.04 to 91.47. The other five architectures also gain accuracy: Top-1 increases by 0.58, 0.15, 0.70, 0.74, 0.72, and Top-5 sees corresponding increments of 0.22, 0.11, 0.50, 0.78, 1.62, respectively.

Beyond accuracy, RepL reduces GPU memory usage and shortens per-epoch training time by 10\%-25\% across all models, highlighting its effectiveness on large-scale ImageNet \cite{r4} even for deeper networks. Similarly, experiments on ViTs \cite{r14} with large datasets confirm our method outperforms the existing Skip-Attention \cite{r21} mechanism.

\subsection{Ablation study}
\subsubsection{\textbf{Performance analysis of computing layer usage}}
\begin{table}[t]
\renewcommand{\arraystretch}{0.8}
\caption{Performance comparison on CIFAR-10.}
\label{t3}
\setlength{\tabcolsep}{5pt}
\centering
\scalebox{0.9}{
\setlength{\tabcolsep}{2.0mm}
\begin{tabular}{ccccc}
\toprule
\textbf{Backbone}
& \textbf{Method}
& \textbf{\makecell{Test\\Accuracy\\(\%)}}
& \textbf{\makecell{GPU\\Memory\\(GB)}}
& \textbf{\makecell{Training Time\\(s/epoch)}} \\
\midrule
                             & E2E                        & 93.49±0.29          & 9.31               & 26.19            \\
                             & - 25\% layers              & 92.62±2.01          & 7.07               & 19.54            \\
\multirow{-3}{*}{ResNet-110}  & \cellcolor[HTML]{E6F0FF}+ computing layers & \cellcolor[HTML]{E6F0FF}94.01±0.17 & \cellcolor[HTML]{E6F0FF}7.62 & \cellcolor[HTML]{E6F0FF}20.93 \\
\midrule
                             & E2E                        & 72.77±1.31          & 2.81               & 6.81             \\
                             & - 25\% layers              & 71.13±1.24          & 2.04               & 5.44             \\
\multirow{-3}{*}{ViT-Tiny/8} & \cellcolor[HTML]{E6F0FF}+ computing layers & \cellcolor[HTML]{E6F0FF}73.71±1.08 & \cellcolor[HTML]{E6F0FF}2.08 & \cellcolor[HTML]{E6F0FF}5.65  \\
\bottomrule
\end{tabular}}
\end{table}



\begin{table}[t]
\renewcommand{\arraystretch}{0.8}
\caption{Performance comparison on ImageNet.}
\label{t4}
\centering
\scalebox{0.90}{
\setlength{\tabcolsep}{1.1mm}
\begin{tabular}{cccccc}
\toprule
\textbf{Backbone}
& \textbf{Method}
& \textbf{\makecell{Top-1\\Accuracy\\(\%)}}
& \textbf{\makecell{Top-5\\Accuracy\\(\%)}}
& \textbf{\makecell{GPU\\Memory\\(GB)}}
& \textbf{\makecell{Training\\Time\\(s/epoch)}} \\
\midrule
& E2E & 74.82±1.43 & 91.04±1.33 & 9.21 & 463.23 \\
& - 25\% layers & 72.99±1.82 & 90.12±1.31 & 7.75 & 392.21 \\
\multirow{-3}{*}{ResNet-34} & \cellcolor[HTML]{E6F0FF}+ computing layers & \cellcolor[HTML]{E6F0FF}75.44±1.27 & \cellcolor[HTML]{E6F0FF}91.47±2.01 & \cellcolor[HTML]{E6F0FF}8.06 & \cellcolor[HTML]{E6F0FF}410.53 \\
\midrule
& E2E & 60.23±1.52 & 82.38±1.33 & 12.17 & 357.66 \\
& - 25\% layers & 58.22±0.91 & 81.51±1.22 & 9.49 & 287.55 \\
\multirow{-3}{*}{ViT-Tiny/16} & \cellcolor[HTML]{E6F0FF}+ computing layers & \cellcolor[HTML]{E6F0FF}60.93±1.19 & \cellcolor[HTML]{E6F0FF}82.88±1.07 & \cellcolor[HTML]{E6F0FF}9.59 & \cellcolor[HTML]{E6F0FF}290.15 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[!t]
\renewcommand{\arraystretch}{0.8} 
\caption{Performance comparison on CIFAR-10 with different $k$ setting.}
\label{t5}
\centering
\scalebox{0.9}{
\setlength{\tabcolsep}{2.3mm}
\begin{tabular}{ccccc}
\toprule
\textbf{Backbone}
& \textbf{$k$ value setting}
& \textbf{\makecell{Test\\Accuracy\\(\%)}}
& \textbf{\makecell{GPU\\Memory\\(GB)}}
& \textbf{\makecell{Training Time\\(s/epoch)}} \\
\midrule
& $k=2$ & 92.67±1.89 & 6.25 & 18.05 \\
& \cellcolor[HTML]{E6F0FF}$k=4$ & \cellcolor[HTML]{E6F0FF}94.01±0.17 & \cellcolor[HTML]{E6F0FF}7.62 & \cellcolor[HTML]{E6F0FF}20.93 \\
\multirow{-3}{*}{ResNet-110} & $k=6$ & 94.11±0.34 & 8.63 & 23.94 \\
\midrule
& $k=2$ & 71.48±2.39 & 1.70 & 5.19 \\
& \cellcolor[HTML]{E6F0FF}$k=4$ & \cellcolor[HTML]{E6F0FF}73.71±1.08 & \cellcolor[HTML]{E6F0FF}2.08 & \cellcolor[HTML]{E6F0FF}5.65 \\
\multirow{-3}{*}{ViT-Tiny/8} & $k=6$ & 73.94±1.17 & 2.39 & 6.39 \\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[!t]
\renewcommand{\arraystretch}{0.8} 
\caption{Ablation of Parameters in Computing Layers.}
\label{tab:repl_ablation}
\centering
\scalebox{0.9}{
\setlength{\tabcolsep}{2.5mm}
\begin{tabular}{lccc}
\toprule
\textbf{Method} 
& \textbf{\makecell{Accuracy\\(\%)}} 
& \textbf{\makecell{GPU\\Memory\\(GB)}} 
& \textbf{\makecell{Training Time\\(sec / epoch)}} \\
\midrule
\cellcolor[HTML]{E6F0FF}RepL & \cellcolor[HTML]{E6F0FF}73.71±1.08 & \cellcolor[HTML]{E6F0FF}2.08 & \cellcolor[HTML]{E6F0FF}5.65 \\
RepL (only Attention weights) & 72.39±0.97 & 2.05 & 5.59 \\
RepL (only MLP weights) & 72.14±1.34 & 2.07 & 5.53 \\
RepL (no weights) & 69.30±2.11 & 2.02 & 5.20 \\
\bottomrule
\end{tabular}}
\end{table}


To demonstrate the necessity of removing certain layers and the role of the computing layer as a replacement, we conduct comparative experiments on the CIFAR-10 \cite{r1} using ViT-Tiny/8 \cite{r14} and ResNet-110 \cite{r5}. The performance of the traditional E2E training \cite{r12}, a network with one-quarter of its layers removed according to the design with \(k=4\), and the network with the insertion of computing layers is evaluated and compared.

As shown in Table \ref{t3} and Table \ref{t4}, after removing 25\% of the layers, there is a significant reduction in GPU memory usage, and the training time is also considerably shortened. This demonstrates the positive impact of layer removal in terms of resource savings and efficiency enhancement. However, this comes at the cost of a decrease in accuracy. To address this limitation, we designed the insertion of computing layers in Replacement Learning to replace the removed layers. The results clearly indicate that our design is effective, as it not only saves GPU memory and reduces training time but also improves accuracy.

\subsubsection{\textbf{Analysis of interval setting for removed layers}}
In the experiments, we set \(k=4\) as the interval for the removed layers. To test the impact of different values of \(k\) on our proposed Replacement Learning, we conduct multiple comparative experiments on the CIFAR-10 \cite{r1} dataset using ViT-Tiny/8 \cite{r14} and ResNet-110 \cite{r5}.

As observed in Table \ref{t5}, when \(k=2\), a larger number of layers are removed, resulting in greater GPU memory savings and a significant reduction in training time. However, this also leads to a reduction in the amount of learned information, which negatively impacts accuracy. When \(k=6\), although the network performs well in terms of performance, it falls short in resource savings. Through comparison, we find that \(k=4\) strikes the best balance between accuracy and resource efficiency.

\subsubsection{\textbf{Comparison of features in different methods}}
\begin{figure*}[!htbp]
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \includegraphics[width=2.4cm]{TPAMI_RepL/sec/bp.png}
  \centerline{(a)}\medskip
\end{minipage}
% \hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \includegraphics[width=2.4cm]{TPAMI_RepL/sec/rl.png}
  \centerline{(b)}\medskip
\end{minipage}
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \includegraphics[width=2.4cm]{TPAMI_RepL/sec/bp2.png}
  \centerline{(c)}\medskip
\end{minipage}
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \includegraphics[width=2.4cm]{TPAMI_RepL/sec/rl2.png}
  \centerline{(d)}\medskip
\end{minipage}
\caption{Visualization of feature maps. (a) Feature map of ResNet-32 with End-to-End training. (b) Feature map of ResNet-32 with Replacement Learning. (c) Feature map of ViT-Tiny/8 with End-to-End training. (d) Feature map of ViT-Tiny/8 with Replacement Learning.} 
\label{f3} 
\end{figure*}

\begin{table*}[t]
\renewcommand{\arraystretch}{0.8} 
\caption{Performance comparison on CIFAR-10 using different layers.}
\label{t6}
\centering
\scalebox{1.0}{
\setlength{\tabcolsep}{7.2mm}
\begin{tabular}{ccc|ccc}
\toprule
\multicolumn{3}{c|}{ResNet-110}                                                                                                               & \multicolumn{3}{c}{ViT-Tiny/8}                                                                                                                \\ \midrule
\begin{tabular}[c]{@{}c@{}}Preceding\\ Layer\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succeeding\\ Layer\end{tabular} & Test Accuracy (\%)  & \begin{tabular}[c]{@{}c@{}}Preceding\\ Layer\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succeeding\\ Layer\end{tabular} & Test Accuracy (\%)  \\ \midrule
\ding{55}                                                          & \ding{55}                                                          & 93.49±0.29          & \ding{55}                                                           & \ding{55}                                                           & 72.77±1.31          \\
\ding{55}                                                           & \ding{51}                                                           & 93.19±1.38          & \ding{55}                                                           & \ding{51}                                                          & 72.18±1.93          \\
\ding{51}                                                          & \ding{55}                                                           & 91.75±2.31          & \ding{51}                                                          & \ding{55}                                                           & 69.37±4.85          \\ \rowcolor[HTML]{E6F0FF}
\textbf{\ding{51}}                                                 & \textbf{\ding{51}}                                                 & \textbf{94.01±0.17} & \textbf{\ding{51}}                                                 & \textbf{\ding{51}}                                                 & \textbf{73.71±1.08} \\ \bottomrule
\end{tabular}}
\end{table*}

To showcase the advanced and distinctive capabilities of Replacement Learning, we conduct feature map analyses on CIFAR-10 \cite{r1} with ResNet-32 \cite{r5}. The corresponding visualization results can be found in Figure \ref{f3}. 

Upon analyzing them, we can observe that (a) and (c), which use End-to-End training, are concentrated in specific regions, indicating the presence of significant information within those areas. Conversely, after using Replacement Learning, (b) and (d) capture more comprehensive global features, including localized edge features. It follows that our method can compensate for the shortcomings of other methods.

\subsubsection{\textbf{Comparison of using different parts of parameters}}
To further validate the critical importance of leveraging the parameters from preceding and succeeding layers, we design and conduct an ablation study. Following the main experimental setup, we use ViT-T/8 as the backbone on the CIFAR-10 dataset. Specifically, we compare the results under four configurations: (i) using both attention parameters (including the qkv and $W_o$ layers) and MLP parameters, (ii) using only attention parameters, (iii) using only MLP parameters, and (iv) not using any parameters from adjacent layers. The ablation results summarized in Table \ref{tab:repl_ablation} clearly indicate that incorporating more parameters consistently leads to better performance. Moreover, attention parameters contribute more significantly than MLP parameters, while excluding all parameters causes a substantial performance drop.

\subsubsection{\textbf{Comparison of using different layers}}
To comprehensively validate effectiveness of our design, we conduct experiments with ResNet-110 \cite{r5}, and ViT-Tiny/8 \cite{r14} as the backbones, using End-to-End training \cite{r12} as the baseline, and comparing three methods for the computing layers: outputs from the preceding layer, outputs from the succeeding layer, and outputs from both the preceding and succeeding layers.

As shown in Table \ref{t6}, when using only the outputs from either the previous or the subsequent layer, there is a noticeable decline in accuracy. In contrast, utilizing both the preceding and succeeding layers simultaneously enhances the model's performance, surpassing that of traditional End-to-End training \cite{r12}. This demonstrates the importance of balancing historical and new information in the design of Replacement Learning, which has a positive impact on model performance.

\subsection{Analytical experiments}

%=====================================================================
\subsubsection{\textbf{Empirical analysis}}
%=====================================================================

\paragraph{Detection experiments and analysis}
To evaluate the performance of Replacement Learning on other tasks, we conduct experiments on the COCO dataset \cite{r51} using RetinaNet-R50 and RetinaNet-R101 \cite{r52} as backbones. In these experiments, we utilize 4 Nvidia A100 GPUs, with a batch size of 8, a learning rate of 4e-5, and the Adam optimizer. The training is carried out for a total of 100 epochs. Detailed results can be found in Table \ref{t7}.

The table illustrates that the Replacement Learning model demonstrates significant performance improvements across various depth detection models, while concurrently reducing both GPU memory usage and training time. These results underscore the effectiveness and efficiency of the proposed method, confirming its versatility in addressing a broad spectrum of deep learning tasks with diverse requirements.

\begin{table*}[!t]
\renewcommand{\arraystretch}{0.8} 
\caption{Performance comparison on COCO using different backbones. * means the addition of Replacement Learning.}
\label{t7}
\centering
\scalebox{1.0}{
\setlength{\tabcolsep}{4.9mm}
\begin{tabular}{cccccc}
\toprule
\textbf{Backbone} & \textbf{mAP} & \textbf{AP@50} & \textbf{AP@75} & \textbf{GPU Memory (GB)} & \textbf{Training Time (s/epoch)} \\ \midrule
RetinaNet-R50     & 30.42        & 51.72          & 30.80          & 6.85                                                               & 3859.11                                                                 \\
\rowcolor[HTML]{E6F0FF} 
RetinaNet-R50*    & 30.64(↑0.22) & 52.44(↑0.72)   & 31.15(↑0.35)   & 5.82(↓15.04\%)                                                     & 3245.23(↓15.91\%)                                                      \\
RetinaNet-R101    & 32.36        & 54.21          & 32.91          & 8.19                                                               & 5548.09                                                                 \\
\rowcolor[HTML]{E6F0FF} 
RetinaNet-R101*   & 32.76(↑0.40) & 54.80(↑0.59)   & 32.98(↑0.07)   & 6.65(↓18.80\%)                                                     & 4671.33(↓15.80\%)                                                      \\ \bottomrule
\end{tabular}}
\end{table*}

\paragraph{Comparison of the distribution of classified data points}
\begin{figure}[h]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=4.5cm]{TPAMI_RepL/sec/tsne2.png}
  \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=4.5cm]{TPAMI_RepL/sec/tsne1.png}
  \centerline{(b)}\medskip
\end{minipage}
\end{center}
\caption{T-SNE visualization. (a) is t-SNE of E2E training, (b) is t-SNE of Replacement Learning.}
\label{fig:tsne}
\end{figure}
To compare E2E Training \cite{r12} and Replacement Learning in feature learning, we perform t-SNE visualization \cite{r50} on ResNet-110 \cite{r5} using the SVHN dataset \cite{r2}, as shown in Figure \ref{fig:tsne}. In the t-SNE plot for End-to-End training (a), significant overlap between target and non-target classes indicates poor class discrimination. In contrast, the Replacement Learning visualization (b) shows more compact and distinct target class clusters, with clearer boundaries between target and non-target classes, reducing inter-class confusion. These results demonstrate the superior classification performance of Replacement Learning over End-to-End training \cite{r12}.

\paragraph{Comparative experiments with related methods}
To verify the generality of our approach, we compare it against Stochastic Depth \cite{sd}, Checkpointing \cite{checkpointing}, and further combine our method with these two techniques. The experimental results are illustrated in the following Table. \ref{tab:repl_sd_ckpt}.

\begin{table}[ht]
\caption{Comparative Experiments with Stochastic Depth and Checkpointing, the results in the table are based on a single run.}
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.9}{
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{@{}lllccc@{}}
\toprule
\textbf{Dataset} & \textbf{Backbone} & \textbf{Method} & \textbf{Acc@1}
& \textbf{\makecell{GPU\\Memory\\(GB)}}
& \textbf{\makecell{Time\\(s/epoch)}} \\
\midrule
\multirow{6}{*}{CIFAR-10} & \multirow{6}{*}{ResNet-32} & E2E                         & 93.17 & 3.38  & 10.44 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL               & \cellcolor[HTML]{E6F0FF}93.43 & \cellcolor[HTML]{E6F0FF}2.69  & \cellcolor[HTML]{E6F0FF}8.20 \\
                          &                               & Stochastic Depth            & 93.04 & 3.31  & 10.05 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL+Stochastic Depth     & \cellcolor[HTML]{E6F0FF}93.17 & \cellcolor[HTML]{E6F0FF}2.67  & \cellcolor[HTML]{E6F0FF}9.36 \\
                          &                               & Checkpointing               & 93.13 & 1.77  & 16.44 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL+Checkpointing        & \cellcolor[HTML]{E6F0FF}93.24 & \cellcolor[HTML]{E6F0FF}1.64  & \cellcolor[HTML]{E6F0FF}14.54 \\
\midrule
\multirow{6}{*}{ImageNet} & \multirow{6}{*}{ResNet-101}  & E2E                         & 77.55 & 20.95 & 720 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL               & \cellcolor[HTML]{E6F0FF}78.13 & \cellcolor[HTML]{E6F0FF}18.01 & \cellcolor[HTML]{E6F0FF}616 \\
                          &                               & Stochastic Depth            & 77.63 & 19.39 & 652 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL+Stochastic Depth     & \cellcolor[HTML]{E6F0FF}78.11 & \cellcolor[HTML]{E6F0FF}17.12 & \cellcolor[HTML]{E6F0FF}551 \\
                          &                               & Checkpointing               & 78.25 & 14.47 & 1012 \\
                          &                               & \cellcolor[HTML]{E6F0FF}RepL+Checkpointing         & \cellcolor[HTML]{E6F0FF}78.29 & \cellcolor[HTML]{E6F0FF}12.93 & \cellcolor[HTML]{E6F0FF}819 \\
\bottomrule
\end{tabular}}
\label{tab:repl_sd_ckpt}
\end{table}

\paragraph{Experiments on the NLP task}
We conduct the experiments on the NLP model, and the experimental configuration and results are shown in the table \ref{nlp} below. The tokenization method adopts basic English tokenization. In the process of building the vocabulary, only words with an occurrence frequency of no less than 2 are retained. Meanwhile, the $<$eos$>$ token is appended at the end of each sentence. For sequence segmentation, the backpropagation through time with a length of 128 is used. The experiment is trained for 20 epochs, and the significant variance is obtained through 5 experiments (different seeds).

\begin{table*}[htbp]
\renewcommand{\arraystretch}{0.8} 
\caption{Performance on WikiText-2 using Transformer-LM-12L-512d-8H-2048ff.}
\label{nlp}
\centering
\scalebox{1.0}{
\setlength{\tabcolsep}{5.7mm}
\begin{tabular}{cclclc}
\toprule
\textbf{Dataset}             & \textbf{Model}                                                                                 & \multicolumn{1}{c}{\textbf{Method}}              & \textbf{Test PPL (↓)}                                      & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}GPU Memory\\ (GB)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time\\ (s/epoch)\end{tabular}} \\ \midrule
                             &                                                                                                & \multicolumn{1}{c}{E2E}                          & \cellcolor[HTML]{FFFDFA}{\color[HTML]{333333} 195.42±1.84} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFDFA}{\color[HTML]{333333} 10.92}}               & \cellcolor[HTML]{FFFDFA}{\color[HTML]{333333} 20.8}                      \\ \cline{3-6} 
\multirow{-2}{*}{WikiText-2} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-LM-12L-512d-8H-2048ff\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{E6F0FF}RepL} & \cellcolor[HTML]{E6F0FF}{\color[HTML]{333333} 193.31±3.39} & \multicolumn{1}{c}{\cellcolor[HTML]{E6F0FF}{\color[HTML]{333333} 9.61}}                & \cellcolor[HTML]{E6F0FF}{\color[HTML]{333333} 17.7}                      \\ \midrule
\multicolumn{2}{c}{}                                                                                                          & \multicolumn{2}{l}{Hardware: Single A100}                                                                     & \multicolumn{2}{l}{Grad\_clip: 1.0}                                                                                                                               \\
\multicolumn{2}{c}{}                                                                                                          & \multicolumn{2}{l}{Batch size: 64}                                                                            & \multicolumn{2}{l}{Weight decay: 0.01}                                                                                                                            \\
\multicolumn{2}{c}{}                                                                                                          & \multicolumn{2}{l}{Optimizer: AdamW}                                                                          & \multicolumn{2}{l}{fp: 16}                                                                                                                                        \\
\multicolumn{2}{c}{\multirow{-4}{*}{Configuration}}                                                                           & \multicolumn{2}{l}{Learning rate: 3e-4}                                                                       &                                                                                        & \multicolumn{1}{l}{}                                                     \\ \bottomrule
\end{tabular}}
\end{table*}

\paragraph{Inference on ImageNet}
We have conducted experiments on inference throughput, and the results are presented in the Table. \ref{tab:imagenet_repl_small}. We use a single GPU, and the batch size is 128.

\begin{table}[htbp]
\caption{Results on the GPU Memory Usage and Time during inference on ResNet-101 and ViT-S/16.}
\centering
\scalebox{1.0}{
\setlength{\tabcolsep}{3.0mm}
\begin{tabular}{lllcc}
\toprule
\textbf{Dataset} & \textbf{Backbone} & \textbf{Method} 
& \textbf{\makecell{GPU\\Memory\\(GB)}} 
& \textbf{\makecell{Time\\(s/epoch)}} \\
\midrule
\multirow{4}{*}{ImageNet} 
  & \multirow{2}{*}{ResNet-101} & E2E  & 3.97 & 39.12 \\
  &                              & \cellcolor[HTML]{E6F0FF}RepL & \cellcolor[HTML]{E6F0FF}3.65 & \cellcolor[HTML]{E6F0FF}36.26 \\
  \cline{2-5}
  & \multirow{2}{*}{ViT-S/16}    & E2E  & 2.69 & 48.29 \\
  &                              & \cellcolor[HTML]{E6F0FF}RepL & \cellcolor[HTML]{E6F0FF}2.45 & \cellcolor[HTML]{E6F0FF}41.42 \\
\bottomrule
\end{tabular}}
\label{tab:imagenet_repl_small}
\end{table}

\paragraph{Fine-tuning on ViTs}
To verify the effectiveness of RepL in the finetuning setting, we conduct experiments on CIFAR-10 \cite{r1}, SVHN \cite{r2}, and STL-10 \cite{r3} using pretrained weights obtained from ImageNet-1K \cite{r4}. The experimental settings are: batch size = 512, learning rate = 2e-4, optimizer = AdamW, and epochs = 100. The results are summarized in Table \ref{tab:finetune}.

\begin{table}[htbp]
\caption{Finetune results on ViT-S/16.}
\label{tab:finetune}
\centering
\scalebox{1.0}{
\setlength{\tabcolsep}{2.1mm}
\begin{tabular}{lllccc}
\toprule
\textbf{Datasets} & \textbf{Model} & \textbf{Method} & \textbf{Acc@1} 
& \textbf{\makecell{GPU\\Memory\\(GB)}} 
& \textbf{\makecell{Time\\(s/epoch)}} \\
\midrule
\multirow{2}{*}{CIFAR-10} & \multirow{2}{*}{ViT-S/16} & E2E   & 95.66 & 25.56 & 32.45 \\
                          &                            & \cellcolor[HTML]{E6F0FF}RepL  & \cellcolor[HTML]{E6F0FF}95.89 & \cellcolor[HTML]{E6F0FF}20.14 & \cellcolor[HTML]{E6F0FF}25.18 \\
\midrule
\multirow{2}{*}{SVHN}     & \multirow{2}{*}{ViT-S/16} & E2E   & 96.92 & 25.56 & 48.44 \\
                          &                            & \cellcolor[HTML]{E6F0FF}RepL  & \cellcolor[HTML]{E6F0FF}96.97 & \cellcolor[HTML]{E6F0FF}20.14 & \cellcolor[HTML]{E6F0FF}38.01 \\
\midrule
\multirow{2}{*}{STL-10}   & \multirow{2}{*}{ViT-S/16} & E2E   & 94.88 & 25.56 & 5.91 \\
                          &                            & \cellcolor[HTML]{E6F0FF}RepL  & \cellcolor[HTML]{E6F0FF}95.11 & \cellcolor[HTML]{E6F0FF}20.14 & \cellcolor[HTML]{E6F0FF}4.66 \\
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Fine-tuning for downstream tasks}
We fine-tune the pre-trained model (ImageNet-1k \cite{r4}, trained with RepL) on the CityScapes dataset using the SGD optimizer with a batch size of 16, a learning rate of 0.1, a crop size of 768, and trained for 30k iterations (about 164 epochs) on a single GPU. The experimental results are shown in the following table \ref{fine tune}.

When fine-tuning for downstream tasks, RepL does not compromise transfer learning performance. First, its computational layers preserve the core feature patterns acquired by the model through parameter fusion of adjacent layers, rather than randomly pruning information. Second, parameter reduction mitigates overfitting risks during fine-tuning, particularly evident in low-data scenarios. Finally, learnable blocks dynamically adjust the weight contributions between preceding and succeeding layers during fine-tuning, enhancing task-specific feature representation.

\begin{table}[h]
\caption{Performance comparison on CityScapes using different backbones.}
\label{fine tune}
\centering
\setlength{\tabcolsep}{0.7pt}
\begin{tabular}{ccccccc}
\toprule
\textbf{Backbone}                    
& \textbf{Method}              
& \textbf{\makecell{Overall\\Accuracy}} 
& \textbf{\makecell{Mean\\Accuracy}} 
& \textbf{\makecell{Mean\\IoU}}                                    
& \textbf{\makecell{GPU\\Memory\\(GB)}} 
& \textbf{\makecell{Time\\(s/epoch)}} \\ 
\midrule
                                     
& E2E                          
& \cellcolor[HTML]{FFFDFA}95.27                
& \cellcolor[HTML]{FFFDFA}80.83             
& \cellcolor[HTML]{FFFDFA}73.34 
& \cellcolor[HTML]{FFFDFA}23.90               
& \cellcolor[HTML]{FFFDFA}80                        
\\
\multirow{-2}{*}{DeepLabV3-R50}      
& \cellcolor[HTML]{E6F0FF}RepL 
& \cellcolor[HTML]{E6F0FF}95.32                
& \cellcolor[HTML]{E6F0FF}81.14             
& \cellcolor[HTML]{E6F0FF}73.81 
& \cellcolor[HTML]{E6F0FF}20.28               
& \cellcolor[HTML]{E6F0FF}68                        
\\ 
\midrule
                                     
& E2E                          
& \cellcolor[HTML]{FFFDFA}95.66                
& \cellcolor[HTML]{FFFDFA}81.89             
& \cellcolor[HTML]{FFFDFA}74.61 
& \cellcolor[HTML]{FFFDFA}26.81               
& \cellcolor[HTML]{FFFDFA}82                        
\\
\multirow{-2}{*}{DeepLabV3Plus-R50}  
& \cellcolor[HTML]{E6F0FF}RepL 
& \cellcolor[HTML]{E6F0FF}95.71                
& \cellcolor[HTML]{E6F0FF}82.21             
& \cellcolor[HTML]{E6F0FF}75.25 
& \cellcolor[HTML]{E6F0FF}22.67               
& \cellcolor[HTML]{E6F0FF}69                        
\\ 
\midrule
                                     
& E2E                          
& \cellcolor[HTML]{FFFDFA}95.51                
& \cellcolor[HTML]{FFFDFA}82.31             
& \cellcolor[HTML]{FFFDFA}74.41 
& \cellcolor[HTML]{FFFDFA}30.91               
& \cellcolor[HTML]{FFFDFA}95                        
\\
\multirow{-2}{*}{DeepLabV3-R101}     
& \cellcolor[HTML]{E6F0FF}RepL 
& \cellcolor[HTML]{E6F0FF}95.54                
& \cellcolor[HTML]{E6F0FF}82.71             
& \cellcolor[HTML]{E6F0FF}74.55 
& \cellcolor[HTML]{E6F0FF}25.90               
& \cellcolor[HTML]{E6F0FF}82                        
\\ 
\midrule
                                     
& E2E                          
& \cellcolor[HTML]{FFFDFA}95.84                
& \cellcolor[HTML]{FFFDFA}83.24             
& \cellcolor[HTML]{FFFDFA}75.53 
& \cellcolor[HTML]{FFFDFA}34.42               
& \cellcolor[HTML]{FFFDFA}101                       
\\
\multirow{-2}{*}{DeepLabV3Plus-R101} 
& \cellcolor[HTML]{E6F0FF}RepL 
& \cellcolor[HTML]{E6F0FF}95.89                
& \cellcolor[HTML]{E6F0FF}84.02             
& \cellcolor[HTML]{E6F0FF}76.31 
& \cellcolor[HTML]{E6F0FF}28.92               
& \cellcolor[HTML]{E6F0FF}86                        
\\ 
\bottomrule
\end{tabular}
\end{table}

\paragraph{Adaptive replacement strategy (Adaptive-RepL)}
To test whether learning where to replace blocks (i.e., an adaptive replacement pattern / adaptive-$k$) can improve the accuracy--efficiency trade-off, we implement an adaptive variant of RepL.
Concretely, we pre-attach a computing layer to every internal block (excluding the first and last blocks), so that any internal block can be replaced when selected.
We maintain a binary replacement mask $\mathbf{m}\in\{0,1\}^{n}$ indicating which blocks are replaced in each epoch.
To ensure a fair comparison with Fixed-RepL (periodic replacement with $k=4$), we keep a fixed replacement budget per epoch:
\begin{equation}
    \sum_{i=1}^{n} m_i \;=\; |\mathcal{F}| ,
\end{equation}
where $|\mathcal{F}|$ is the number of replaced sites in Fixed-RepL.
During training, we compute a per-block redundancy/similarity score (measuring how similar neighboring-block representations are),
and update $\mathbf{m}$ by selecting the top-$|\mathcal{F}|$ internal blocks with the highest redundancy scores.
Therefore, the actual replacement locations can change across epochs, instead of being fixed at regular intervals.

\noindent\textbf{Results.}
All hyperparameters are kept identical to the CIFAR-10 settings in the main paper (optimizer, learning-rate schedule, batch size, and epochs).
Table~\ref{tab:adaptive_repl} compares Fixed-RepL and Adaptive-RepL on CIFAR-10.

\begin{table}[t]
\centering
\caption{Comparison between fixed and adaptive replacement strategies on CIFAR-10.}
\renewcommand{\arraystretch}{1.2} 
\label{tab:adaptive_repl}
\scalebox{0.96}{
\setlength{\tabcolsep}{1.1mm}
\begin{tabular}{lllccc}
\toprule
\textbf{Data} & \textbf{Backbone} & \textbf{Method} & \textbf{ACC@1}
& \textbf{\makecell{GPU\\Memory\\(GB)}}
& \textbf{\makecell{Training\\Time\\(s/epoch)}} \\
\midrule
\cellcolor[HTML]{E6F0FF}CIFAR-10 & \cellcolor[HTML]{E6F0FF}ResNet-32  & \cellcolor[HTML]{E6F0FF}Fixed-RepL (Ours) & \cellcolor[HTML]{E6F0FF}93.43 & \cellcolor[HTML]{E6F0FF}2.69 & \cellcolor[HTML]{E6F0FF}8.20 \\
 CIFAR-10 & ResNet-32  & Adaptive-RepL     & 92.54 & 3.17 & 9.12 \\
\cellcolor[HTML]{E6F0FF}CIFAR-10 & \cellcolor[HTML]{E6F0FF}ViT-Tiny/8 & \cellcolor[HTML]{E6F0FF}Fixed-RepL (Ours) & \cellcolor[HTML]{E6F0FF}73.71 & \cellcolor[HTML]{E6F0FF}2.08 & \cellcolor[HTML]{E6F0FF}5.65 \\
CIFAR-10 & ViT-Tiny/8 & Adaptive-RepL     & 71.97 & 2.35 & 6.17 \\
\bottomrule
\end{tabular}}
\end{table}

\noindent\textbf{Why adaptive replacement underperforms.}
As shown in Table~\ref{tab:adaptive_repl}, Adaptive-RepL is consistently worse than Fixed-RepL on both backbones:
(i) it yields lower accuracy (ResNet-32: $-0.89$; ViT-Tiny/8: $-1.74$ ACC@1),
(ii) it requires more GPU memory (ResNet-32: $+0.48$ GB; ViT-Tiny/8: $+0.27$ GB),
and (iii) it is slower per epoch (ResNet-32: $+0.92$ s/ep; ViT-Tiny/8: $+0.52$ s/ep).
We attribute this to three factors:
\textbf{(1) Higher overhead:} pre-attaching computing layers to all internal blocks and maintaining/updating the mask introduces extra computation and memory footprint.
\textbf{(2) Optimization non-stationarity:} changing the replacement positions across epochs makes the effective network topology time-varying, which disrupts stable layer-wise co-adaptation and can hurt convergence.
\textbf{(3) Noisy/early scores:} redundancy scores derived from intermediate representations can be unreliable (especially in early training),
so the adaptive policy may replace critical blocks and thus degrade accuracy.
Overall, the additional complexity of learning replacement locations does not bring better accuracy--efficiency trade-offs, supporting our choice of a simple fixed periodic replacement pattern in the main method.

\paragraph{Extra ablation study on ViT}
In our ViT experiments, RepL employs two learnable parameters, $\alpha$ and $\beta$, to fuse the parameters from the preceding and succeeding layers, respectively. To validate that using two learnable parameters is indeed more effective than a single one, we conducted an ablation study. As shown in the Table. \ref{tab:repl_param_ablation}, introducing both $\alpha$ and $\beta$ does not incur any additional GPU memory consumption or training time. Moreover, this configuration consistently achieves noticeably better performance compared to using a single learnable parameter.

\begin{table}[htbp]
\caption{Ablation on the number of parameters in RepL. We use ViT-T/8 on the CIFAR-10 dataset.}
\centering
\setlength{\tabcolsep}{10pt}
\scalebox{0.96}{
\setlength{\tabcolsep}{3.1mm}
\begin{tabular}{lccc}
\toprule
\textbf{Method} 
& \textbf{\makecell{Accuracy\\(\%)}} 
& \textbf{\makecell{GPU\\Memory\\(GB)}} 
& \textbf{\makecell{Training Time\\(s/epoch)}} \\
\midrule
\cellcolor[HTML]{E6F0FF}RepL(2 parameter) & \cellcolor[HTML]{E6F0FF}$73.71 \pm 1.08$ & \cellcolor[HTML]{E6F0FF}2.08 & \cellcolor[HTML]{E6F0FF}5.65 \\
RepL(1 parameter) & $73.09 \pm 0.85$ & 2.08 & 5.65 \\
\bottomrule
\end{tabular}}
\label{tab:repl_param_ablation}
\end{table}

\paragraph{RepL is orthogonal to deployment-time quantization}
\label{sec:repl_quantization}
To further verify that RepL is orthogonal to deployment-time inference optimizations, we conduct post-hoc INT8 quantization on ImageNet-1K \cite{r4} for both ViT-S/16 \cite{r14} and ResNet-34 \cite{r5}.
For ViTs \cite{r14}, we apply dynamic INT8 quantization to linear layers (\texttt{int8\_dynamic\_linear}); for ResNets, we use FX graph-mode static quantization (\texttt{int8\_fx\_static}) with calibration.
Table~\ref{tab:repl_quant_imagenet} reports Top-1/Top-5 accuracy as well as the measured throughput/latency from our reference implementation.

\begin{table*}[htbp]
\centering
\small
\setlength{\tabcolsep}{11pt}
\renewcommand{\arraystretch}{1.05}
\caption{\textbf{Post-hoc INT8 quantization on ImageNet-1K.}
ViT \cite{r14} uses dynamic INT8 quantization on linear layers (\texttt{int8\_dynamic\_linear}); ResNet \cite{r5} uses FX graph-mode static INT8 quantization with calibration (\texttt{int8\_fx\_static}).
$\Delta$ denotes INT8 minus FP32. Throughput is measured in img/s and latency in ms/img.}
\label{tab:repl_quant_imagenet}
\begin{tabular}{l c cc cc cc cc}
\toprule
Backbone & Method &
\multicolumn{2}{c}{FP32 Acc. (\%)} &
\multicolumn{2}{c}{INT8 Acc. (\%)} &
$\Delta$Top-1 & $\Delta$Top-5 &
FP32 & INT8 \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
& & Top-1 & Top-5 & Top-1 & Top-5 & (\%) & (\%) & (img/s) & (img/s) \\
\midrule
ViT-S/16  & BP   & 63.760 & 83.864 & 63.242 & 83.290 & -0.518 & -0.574 & 1022.948 & 45.788 \\
\cellcolor[HTML]{E6F0FF}ViT-S/16  & \cellcolor[HTML]{E6F0FF}RepL & \cellcolor[HTML]{E6F0FF}65.336 & \cellcolor[HTML]{E6F0FF}85.766 & \cellcolor[HTML]{E6F0FF}64.222 & \cellcolor[HTML]{E6F0FF}84.534 & \cellcolor[HTML]{E6F0FF}-1.114 & \cellcolor[HTML]{E6F0FF}-1.232 & \cellcolor[HTML]{E6F0FF}1072.901 & \cellcolor[HTML]{E6F0FF}48.723 \\
ResNet-34 & BP   & 73.660 & 91.152 & 73.496 & 91.086 & -0.164 & -0.066 & 1757.045 & 194.469 \\
\cellcolor[HTML]{E6F0FF}ResNet-34 & \cellcolor[HTML]{E6F0FF}RepL & \cellcolor[HTML]{E6F0FF}75.112 & \cellcolor[HTML]{E6F0FF}91.914 & \cellcolor[HTML]{E6F0FF}74.832 & \cellcolor[HTML]{E6F0FF}91.710 & \cellcolor[HTML]{E6F0FF}-0.280 & \cellcolor[HTML]{E6F0FF}-0.204 & \cellcolor[HTML]{E6F0FF}1837.255 & \cellcolor[HTML]{E6F0FF}249.975 \\
\bottomrule
\end{tabular}

\vspace{0.35em}
\footnotesize
\textbf{Latency (ms/img).}
ViT-S/16 BP: FP32 0.978, INT8 21.839; \ \ ViT-S/16 RepL: FP32 0.932, INT8 20.524.
ResNet-34 BP: FP32 0.569, INT8 5.142; \ \ ResNet-34 RepL: FP32 0.544, INT8 4.000.
\end{table*}

\noindent\textbf{Discussion.}
First, RepL weights can be directly quantized using standard PyTorch post-training quantization pipelines (dynamic for ViT, FX static for ResNet), indicating strong compatibility with deployment-time quantization.
Second, RepL consistently improves absolute accuracy under both FP32 and INT8:
for ViT-S/16, RepL is +1.576 Top-1 / +1.902 Top-5 in FP32 and still +0.980 Top-1 / +1.244 Top-5 after INT8;
for ResNet-34, RepL is +1.452 Top-1 / +0.762 Top-5 in FP32 and +1.336 Top-1 / +0.624 Top-5 after INT8.
Finally, INT8 introduces only a small accuracy degradation for both BP and RepL (within 1.2\% Top-1 in all cases), suggesting that the gains from RepL remain largely preserved after quantization.



%=====================================================================
% \subsubsection{\textbf{Theoretical analysis}}
% %=====================================================================

% \paragraph{Parameter analysis}
% \label{param}
% We quantify how many learnable weights are discarded by Replacement Learning and how many new ones are introduced. Let a network contain $n$ layers, indexed from $1$ to $n$.
% Denote by $P_i:=\lVert W_{i}\rVert_{0}$ the number of parameters of the $i$-th layer,\footnote{For CNNs $P_i=C^{\text{out}}_{i}C^{\text{in}}_{i}
% k^{2}$; for ViTs, it is the sum of the projection matrices of the $i$-th transformer block.} and let
% \(
% P_{\text{tot}}^{\text{E2E}}
%   :=\sum_{i=1}^{n} P_i
% \)
% be the parameter count of ordinary end-to-end training.

% \noindent\textbf{Replacement Learning with removal interval $k$.}\;
% A fraction
% \(
% \gamma :=\lvert\mathcal{F}\rvert/n
%          =\bigl\lfloor \frac{n}{k}\bigr\rfloor/n
%          \approx \frac{1}{k}
% \)
% of the layers are removed.  
% The \emph{retained} parameters are therefore
% \(
% (1-\gamma)\,P_{\text{tot}}^{\text{E2E}}.
% \)

% \textbf{CNNs.}
% For every removed layer $i\!\in\!\mathcal{F}$ two depth-wise $1{\times}1$ convolutions are inserted, contributing
% \begin{equation}
%   \underbrace{C^{\text{out}}_{i-1}}_{\phi_{i-1}}+
%   \underbrace{C^{\text{out}}_{i+1}}_{\phi_{i+1}}
%   \quad\text{weights}.
% \end{equation}

% \noindent \emph{Upper bound.}
% Because $C^{\text{out}}_{i\pm1}\le
% \max_{j} C^{\text{out}}_{j}$, the total number of \emph{new} weights satisfies
% \begin{equation}
%   P_{\text{add}}^{\text{CNN}}
%   \;\le\;
%   2\,\gamma n\,
%   \max_{j}C^{\text{out}}_{j}
%   \;=\;
%   \tfrac{2n}{k}\;
%   C_{\max}.
% \end{equation}

% Since a normal $k{\times}k$ convolution carries
% $C^{\text{out}}_{i}C^{\text{in}}_{i}k^{2}$ parameters, one obtains the \emph{global} bound
% \begin{equation}
% \begin{aligned}
%   P_{\text{tot}}^{\text{RepL}}
%   &\le (1-\gamma)\,P_{\text{tot}}^{\text{E2E}} +\tfrac{2n}{k}\,C_{\max} \\
%   &< \Bigl(1-\tfrac{1}{k}\Bigr)\,P_{\text{tot}}^{\text{E2E}} + \mathcal{O}\!\bigl(nC_{\max}\bigr).
% \end{aligned}
% \label{eq:param_upper_cnn}
% \end{equation}

% \textbf{ViTs.}
% Each removed transformer block contributes exactly two learnable parameters, hence
% \begin{equation}
%   P_{\text{add}}^{\text{ViT}} = 2\,\gamma n = \tfrac{2n}{k},
%   \qquad
%   P_{\text{tot}}^{\text{RepL}}
%   =(1-\gamma)\,P_{\text{tot}}^{\text{E2E}} + \tfrac{2n}{k}.
%   \label{eq:param_vit}
% \end{equation}

% \textbf{Tightness.}
% If all $P_i$ are identical ($P_i\equiv\bar{P}$) one has
% $P_{\text{tot}}^{\text{E2E}}=n\bar P$ and
% \(
% P_{\text{tot}}^{\text{RepL}}
%    =(1-\gamma)n\bar P+P_{\text{add}},
% \)
% so the relative reduction is bounded by
% \begin{equation}
%   \frac{P_{\text{tot}}^{\text{RepL}}}{P_{\text{tot}}^{\text{E2E}}}
%   = 1 - \frac{1}{k}
%     + \mathcal{O}\!\Bigl(\frac{1}{n}\Bigr)
%   \;
%   \qquad
%   (\text{CNN \& ViT}).
% \end{equation}

% Thus, Replacement Learning discards \emph{at least} $\frac{1}{k}$ of the original parameters and its overhead decays as $n$ grows.

% \paragraph{Complexity analysis}
% \label{comp}
% We analyse the change in \emph{floating-point operations} (FLOPs) and
% \emph{activation memory} during one training iteration.

% \noindent\textbf{FLOPs.}
% \textbf{CNNs.}
% A standard $k{\times}k$ convolution with stride~1 on a feature map of size $H\times W$
% costs
% \begin{equation}
%   F_{\text{conv}} = 2\,C^{\text{in}}\,C^{\text{out}}\,k^{2}\,HW.
% \end{equation}
% At a replaced site, the learnable blocks $\mathcal{T}_{i-1},\mathcal{T}_{i+1}$ act in \emph{weight
% space} and introduce no per-pixel cost. At run time, we apply a single $1{\times}1$
% convolution $\widehat{W}_i\!\in\!\mathbb{R} ^{C^{\text{in}}_{i+1}\times C^{\text{in}}_{i-1}\times1\times1}$:
% \begin{equation}
%   F_{\text{RepL}}^{\text{CNN}} \;=\; 2\,C^{\text{in}}_{i-1}\,C^{\text{in}}_{i+1}\,HW.
% \end{equation}
% Since $k>1$ and typically $C^{\text{in}}_{i\pm1}\!\approx\!C^{\text{out}}_{i\pm1}$,
% \begin{equation}
%   \frac{F_{\text{RepL}}^{\text{CNN}}}{F_{\text{conv}}}
%   \;=\; \frac{C^{\text{in}}_{i-1}\,C^{\text{in}}_{i+1}}{C^{\text{in}}_{i}\,C^{\text{out}}_{i}\,k^{2}}
%   \;\le\; \frac{1}{k^{2}}.
% \end{equation}
% Replacing a fraction $\gamma\!\approx\!\frac{1}{k}$ of blocks yields the network-level bound
% \begin{equation}
%   F_{\text{tot}}^{\text{RepL}}
%   \;\le\;
%   \bigl(1-\gamma\bigr)\,F_{\text{tot}}^{\text{E2E}}
%   \;+\;\gamma\,\tfrac{1}{k^{2}}\,F_{\text{tot}}^{\text{E2E}}
%   \;=\;
%   \Bigl(1-\tfrac{1}{k}+\tfrac{1}{k^{3}}\Bigr)\,F_{\text{tot}}^{\text{E2E}}.
%   \label{eq:flop_bound_cnn_fixed}
% \end{equation}

% \textbf{ViTs.}
% Let a standard transformer block cost $F_{\text{SA}}$ FLOPs (self-attention $+$ MLP).
% At a replaced site, the learnable block is implemented by two scalars $(\alpha_i,\beta_i)$
% and executes only two $d{\times}d$ linear maps on all $T$ tokens:
% \begin{equation}
%   F_{\text{RepL}}^{\text{ViT}} \;=\; 2\cdot (2d^{2}T) \;=\; 4d^{2}T,
% \end{equation}
% thus
% \begin{equation}
%   F_{\text{tot}}^{\text{RepL}}
%   \;\le\;
%   \bigl(1-\gamma\bigr)\,F_{\text{tot}}^{\text{E2E}}
%   \;+\;\gamma\cdot \frac{4d^{2}T}{F_{\text{SA}}}\,F_{\text{tot}}^{\text{E2E}}
%   \;<\;
%   \Bigl(1-\tfrac{1}{k}\Bigr)\,F_{\text{tot}}^{\text{E2E}},
%   \label{eq:flop_bound_vit_fixed}
% \end{equation}
% because $F_{\text{SA}}\!\gg\!4d^{2}T$ in practice.

% \noindent\textbf{Activation / Memory Footprint.}
% During training, removing a convolutional or transformer block also removes its
% checkpointed \emph{input} activation for backprop. Let $A_i$ be the size (bytes)
% of the input activation to block $i$. The E2E peak is
% $M^{\text{E2E}}_{\text{peak}}=\max_{i}\sum_{j\le i}A_j$.
% RepL discards every $k$-th block from the executed path; the learnable blocks act
% in weight space and add no extra feature maps. Hence
% \begin{equation}
%   M^{\text{RepL}}_{\text{peak}}
%   \;\le\;
%   \Bigl(1-\tfrac{1}{k}\Bigr)\,M^{\text{E2E}}_{\text{peak}}
%   \;+\; \mathcal{O}\!\Bigl(\tfrac{n}{k}\Bigr)\cdot \underbrace{\text{(LN/BN stats)}}_{\text{negligible}} ,
% \end{equation}
% which is consistent with the empirical $15\%\!-\!26\%$ GPU-memory reduction.

% \textbf{Discussion.}
% Eq.\,(\ref{eq:param_upper_cnn})–(\ref{eq:flop_bound_vit_fixed}) show that, for both CNNs and ViTs, Replacement Learning enjoys \emph{linear} savings in parameters, FLOPs and peak memory with respect to the removal rate $\frac{1}{k}$, while introducing only $\mathcal{O}(\frac{n}{k})$ extra learnable parameters or depth-wise
% kernels. These tight bounds theoretically explain the consistent empirical gains observed across all datasets and model families.

% \paragraph{Error bound \& Convergence analysis}
% \label{sec:error_convergence}
% \noindent\textbf{Additional notation.}  
% Let $F(\mathbf{x};\theta)=f_{n}\!\circ\dots\circ f_{1}(\mathbf{x})$
% be the \emph{baseline} network and  
% $\widehat{F}(\mathbf{x};\theta,\,\psi)$
% its \emph{Replacement Learning} variant,
% where $\psi$ collects all learnable block parameters.
% Denote the loss by 
% $\mathcal{L}(\cdot,y)\!:\mathbb{R}^{d_{\!o}}\!\!\to\!\mathbb{R}$,
% and write
% \(
% \ell(\theta):=\mathbb{E}_{(\mathbf{x},y)}\,
%   \mathcal{L}\!\bigl(F(\mathbf{x};\theta),y\bigr)
% \)
% and
% \(
% \widehat\ell(\theta,\psi):=
%   \mathbb{E}_{(\mathbf{x},y)}\,
%   \mathcal{L}\!\bigl(\widehat{F}(\mathbf{x};\theta,\psi),y\bigr).
% \)

% \noindent\textbf{Approximation bias of a computing layer.}

% \begin{definition}[Local operator deviation]
% Let $g_i(\cdot)$ be the (linear part of the) original block-$i$ map before
% its normalization/nonlinearity, and $\widehat g_i(\cdot)$ be the corresponding
% map produced by the learnable block (i.e., $\widehat g_i(\mathbf{h})=\widehat W_i\mathbf{h}$
% for CNNs and $\widehat g_i(\mathbf{h})=\widehat A_i\mathbf{h} + \widehat M_i\mathbf{h}$ for ViTs).
% Define the operator-norm deviation
% \begin{equation}
%   \varepsilon_i \;:=\;
%   \sup_{\mathbf{h}\neq 0}\frac{\|\widehat g_i(\mathbf{h})-g_i(\mathbf{h})\|}{\|\mathbf{h}\|},\qquad
%   \varepsilon_{\max}=\max_{i\in\mathcal F}\varepsilon_i.
%   \label{eq:op_dev_def}
% \end{equation}
% \end{definition}
% This avoids shape-mismatch issues and subsumes the CNN alignment maps
% $\mathcal{T}_{i\pm1}$ implicitly through $\widehat g_i$.

% \begin{lemma}[Layer-wise output deviation]
% \label{lem:layer_dev_fixed}
% If each block (including its normalization/nonlinearity) is $L$-Lipschitz, then
% for any input $\mathbf{x}$,
% \begin{equation}
%   \bigl\|\widehat F(\mathbf{x};\theta,\psi) - F(\mathbf{x};\theta)\bigr\|
%   \;\le\; L^{|\mathcal F|}\,\varepsilon_{\max}\,\max_{i\in\mathcal F}\|\mathbf{h}_{i-1}\|.
% \end{equation}
% \end{lemma}
% \begin{proof}
% Insert $\widehat g_i=g_i+(\widehat g_i-g_i)$ into the forward recursion at
% replaced sites and propagated Lipschitz bounds.
% \end{proof}

% \noindent\textbf{Gradient bias and stable training.}

% \begin{lemma}[Gradient deviation]%
% \label{lem:grad_dev}
% Let every composite function up to layer $j$
% be $L$-smooth\footnote{%
% $g$ is $L$-smooth if $\Vert\nabla g(a)-\nabla g(b)\Vert\le L\Vert a-b\Vert$.}.
% Then
% \begin{equation}
%   \bigl\|
%     \nabla_{\!\theta}\widehat\ell(\theta,\psi)
%     \;-\;
%     \nabla_{\!\theta}\ell(\theta)
%   \bigr\|
%   \;\le\;
%   L\;H_{\max}\,\varepsilon_{\max}.
%   \label{eq:grad_bias}
% \end{equation}
% \end{lemma}

% \begin{proof}
% Using Lemma \ref{lem:layer_dev_fixed} and $L$-smoothness of the composite
% loss,  
% \(
% \Vert\nabla\mathcal{L}(\widehat{F})-\nabla\mathcal{L}(F)\Vert
% \le L\Vert\widehat{F}-F\Vert.
% \)
% Take the expectation over the data.
% \end{proof}

% \noindent\textbf{Convergence under SGD and Adam.}
% \label{sec:convergence_sgd_adam}
% \textbf{Setup.}
% Let $F(\mathbf{x};\theta)=f_{n}\!\circ\dots\circ f_{1}(\mathbf{x})$ be the baseline network and
% $\widehat{F}(\mathbf{x};\theta,\psi)$ the variant trained with learnable blocks,
% where $\psi$ collects all learnable block parameters.
% Given a sample $(\mathbf{x},y)$ and a loss $\mathcal{L}(\cdot,y)$,
% define the population objectives
% \begin{equation}
% \begin{aligned}
%     \ell(\theta) &:= \mathbb{E}_{(\mathbf{x},y)}\bigl[\mathcal{L}\bigl(F(\mathbf{x};\theta),y\bigr)\bigr], \\[4pt]
%     \widehat{\ell}(\theta,\psi) &:= \mathbb{E}_{(\mathbf{x},y)}\bigl[\mathcal{L}\bigl(\widehat{F}(\mathbf{x};\theta,\psi),y\bigr)\bigr].
% \end{aligned}
% \label{eq:loss_def}
% \end{equation}

% \textbf{Assumptions.}
% We make the following standard conditions used in nonconvex analyses:
% \begin{itemize}
% \item[(A1)] Each $f_j$ is $L$-smooth and $G$-Lipschitz; $\mathcal{L}(\cdot,y)$ is $L$-smooth.
% \item[(A2)] Mini-batch gradients are unbiased with variance $\sigma^2$:
% $\mathbb{E}[g_t]=\nabla \widehat{\ell}(\theta_t,\psi_t)$ and
% $\mathbb{E}\|g_t-\nabla \widehat{\ell}(\theta_t,\psi_t)\|^2\le \frac{\sigma^2}{B}$
% for batch size $B$.
% \item[(A3)] (Bounded synthesis bias) For every removed index $i\in\mathcal{F}$, the learnable-block
% synthesis error on weights is bounded in Frobenius norm by $\varepsilon$; equivalently,
% the \emph{induced} gradient bias satisfies
% $\bigl\|\nabla_{\theta}\widehat{\ell}(\theta,\psi)-\nabla_{\theta}\ell(\theta)\bigr\|\le c\,\varepsilon$
% for some constant $c$ depending on $(L,G)$ (Lemma~\ref{lem:grad-bias}).
% \end{itemize}

% \begin{lemma}[Gradient bias induced by learnable blocks]
% \label{lem:grad-bias}
% Assume the forward discrepancy introduced at the removed sites is bounded as
% $\|\widehat{F}(\mathbf{x};\theta,\psi)-F(\mathbf{x};\theta)\|\le H_{\max}\,\varepsilon$
% for all $(\mathbf{x},y)$, where $H_{\max}$ upper-bounds the relevant activations.
% If $\mathcal{L}(\cdot,y)$ is $L$-smooth, then
% \[
% \bigl\|\nabla_{\!\theta}\widehat{\ell}(\theta,\psi)-\nabla_{\!\theta}\ell(\theta)\bigr\|
% \;\le\; L\,H_{\max}\,\varepsilon.
% \]
% \end{lemma}

% \begin{proof}
% By $L$-smoothness of $\mathcal{L}(\cdot,y)$ and the chain rule,
% $\bigl\|\nabla \mathcal{L}(\widehat{F})-\nabla \mathcal{L}(F)\bigr\|
% \le L\|\widehat{F}-F\|$ pointwise; take expectation and use the assumed forward bound.
% \end{proof}

% \textbf{Bias in practice: empirical $\varepsilon$ via forward and gradient deviations.}
% Our analysis above assumes that
%  $ \big\|\nabla_\theta \ell_b - \nabla_\theta \ell\big\|\le L \cdot H_{\max} \cdot \varepsilon$,
% where $\ell_b$ is the loss under RepL, $\ell$ is the loss under the base network, $H_{\max}$ captures the number of replacements, and $\varepsilon$ summarizes the local approximation error. We now provide a concrete measurement of this bias on the same ViT-tiny / CIFAR-10 setting.

% \textbf{RepL model:}  
% We use the trained RepL ViT-tiny checkpoint on CIFAR-10 \cite{r1} corresponding to the “replace” setting in our main experiments:

% \hspace{2em}depth 12, embedding dimension 192, 3 heads, patch size $8\times 8$;

% \hspace{2em}periodic removal with interval 4, excluding the last block. Under this schedule, there are three replacement sites at depth indices 2, 6, and 10 (0-based).

% \textbf{Training setup (summary).}  
% The RepL ViT-tiny is trained using the same pipeline as the baseline ViT:

% \hspace{2em}optimizer: AdamW with weight decay 0.05;

% \hspace{2em}initial learning rate: $1\times 10^{-3}$ (cosine decay with 5-epoch linear warmup);

% \hspace{2em}batch size: 512;

% \hspace{2em}epochs: 250;

% data augmentations identical to the baseline ViT.

% \textbf{Experimental protocol.} 
% In our implementation, each replacement site is realized by a lightweight computing layer that adds a synthesized residual update (constructed from neighboring blocks) to the hidden representation. For the bias diagnostic, we exploit the fact that the contribution of each computing layer can be scaled continuously; in particular, we can:

% \hspace{2em}set the scale to 0 to effectively disable the replacement contribution at that site (only the skip path remains);

% \hspace{2em}set the scale to 1 to fully enable the replacement contribution at that site.

% Using this mechanism, we define:

% \hspace{2em}$F$: the baseline network, obtained by disabling the replacement contribution at all computing layers (scales set to 0). This corresponds to using only the kept backbone blocks with their trained weights.

% \hspace{2em}$F_b^{(r)}$: the same network where the first $r$ replacement sites (in depth order) are enabled (scale = 1), and the remaining ones are kept disabled (scale = 0), with $r \in \{0,1,2,3\}$. All parameters of the backbone are shared between $F$ and $F_b^{(r)}$.

% For each $r$, we measure two quantities:

% \textbf{Forward deviation on logits:}
% $d_{\mathrm{fwd}}(r) = \mathbb{E}_x \big[ \|F_b^{(r)}(x) - F(x)\|_2 \big]$, where the norm is taken over the class logits for each sample.

% \textbf{Gradient deviation on shared parameters:} $d_{\mathrm{grad}}(r) = \big\|\nabla_\theta \ell_b^{(r)} - \nabla\theta \ell\big\|_2,$ where $\ell$ and $\ell_b^{(r)}$ are the cross-entropy losses of $F$ and $F_b^{(r)}$, and $\theta$ includes all shared parameters (we explicitly exclude the parameters of the computing layers when forming the gradient vector). We also report the normalized ratio $\rho(r) = \frac{d_{\mathrm{grad}}(r)}{\|\nabla_\theta \ell\|_2}.$

% In practice, we estimate these quantities on CIFAR-10 test batches with:

% \hspace{2em}20 batches (batch size 256) to estimate $d_{\mathrm{fwd}}(r)$;

% \hspace{2em}10 batches (batch size 256) to estimate $d_{\mathrm{grad}}(r)$ and $\rho(r)$.

% \textbf{Results.} The measured deviations are:
% \begin{table}[h]
% \renewcommand{\arraystretch}{1.0} 
% \centering
% \caption{Results for deviations on CIFAR-10}
% \scalebox{1.0}{
% \setlength{\tabcolsep}{1.5mm}
% \begin{tabular}{cccc}
% \toprule
% \makecell{Active\\replacements\\$r$}  & $d_{\mathrm{fwd}}(r)$ (mean logit $\ell_2$)        & $d_{\mathrm{grad}}(r)$        & $\rho(r) = \frac{d_{\mathrm{grad}}(r) }{\|\nabla_\theta \ell\|_2}$      \\ \midrule
% 0 & 0.000000 & 0.000000 & 0.0000 \\
% 1 & 1.056977 & 1.467278 & 0.1431 \\
% 2 & 1.093139 & 1.498927 & 0.1491 \\
% 3 & 1.141932 & 1.545640 & 0.1597 \\ \bottomrule
% \end{tabular}}
% \end{table}
% We observe that:
% \begin{enumerate}
%     \item At $r = 0$, we have$ F_b^{(0)} = F$ by construction, so both forward and gradient deviations are exactly zero.
%     \item  When we enable a single replacement site $(r = 1)$, the normalized gradient bias is $\rho(1) \approx \mathbf{0.143}$, i.e., the difference between $\nabla_\theta \ell_b^{(1)}$ and $\nabla_\theta \ell$ is about 14\% of the baseline gradient norm. This indicates a modest and controlled bias in the shared-parameter gradients.
%     \item When we enable two or three replacement sites $(r = 2,3)$, both the forward and gradient deviations increase slowly and smoothly:
%      - $\rho(2) \approx \mathbf{0.149}$,
%      - $\rho(3) \approx \mathbf{0.160}$.
%      The growth from $r = 1$ to $r = 3$ is mild and close to linear in $r$, consistent with our non-expansive composition analysis involving $H_{\max}$.
% \end{enumerate}

% Overall, these diagnostics show that the empirical bias \(\varepsilon\) entering
%  $\big\|\nabla_\theta \ell_b - \nabla_\theta \ell\big\| \le L \cdot H_{\max} \cdot \varepsilon$
% is small (with $\rho(r) < 0.16$ even when all replacement sites are enabled) and grows slowly as more blocks are replaced. This provides direct empirical support that RepL introduces a controlled and modest bias in both forward predictions and shared-parameter gradients in the regimes considered in our experiments.

% \begin{theorem}[SGD convergence with learnable blocks]
% \label{thm:sgd}
% Under (A1)–(A3), run SGD \cite{r8} on $(\theta,\psi)$ with step sizes $\eta_t=\frac{\eta}{\sqrt{t}}$ for $T$ steps.
% Let $\ell^\star:=\inf_{\theta}\ell(\theta)$ and denote the constant
% $\beta:=L\,H_{\max}$ from Lemma~\ref{lem:grad-bias}.
% Then
% \begin{equation}
% \begin{aligned}
% \frac{1}{T}\sum_{t=1}^{T}\mathbb{E}\bigl[\|\nabla \widehat{\ell}(\theta_t,\psi_t)\|^2\bigr]
% \;\le\;
% &\underbrace{\frac{2(\ell_0-\ell^\star)}{\eta\sqrt{TB}}+\frac{\eta L\sigma^2}{B}}_{\text{standard nonconvex SGD~\cite{r53}}} \\
% &\;+\;
% \underbrace{2\,\beta\,\varepsilon}_{\text{bias from learnable blocks}}.
% \end{aligned}
% \label{eq:sgd-bound}
% \end{equation}
% \end{theorem}

% \begin{proof}[Sketch]
% Follow the descent-lemma proof for nonconvex SGD~\cite{ghadimi2013sgd} but write the update in
% terms of the \emph{perturbed} gradient
% $\nabla \widehat{\ell}=\nabla \ell + b$, where $\|b\|\le \beta\,\varepsilon$ by Lemma~\ref{lem:grad-bias}.
% The cross term contributes an additive constant $\mathcal{O}(\beta\varepsilon)$ that telescopes to
% $2\beta\varepsilon$ in the averaged bound, yielding \eqref{eq:sgd-bound}.
% \end{proof}

% \begin{corollary}[Adam/AdamW]
% \label{cor:adam}
% If Adam is used with AMSGrad-style conditions, ensuring convergence in the nonconvex setting
% (e.g., \cite{reddi2018convergence}), or AdamW with standard assumptions, then the iterates satisfy
% \begin{equation}
%     \min_{1\le t\le T}\;
% \mathbb{E}\bigl[\|\nabla \widehat{\ell}(\theta_t,\psi_t)\|^2\bigr]
% \;=\;
% \widetilde{\mathcal{O}}\!\bigl(T^{-\frac{1}{2}}\bigr)
% \;+\;
% \mathcal{O}(\varepsilon),
% \end{equation}
% i.e., the usual $T^{-\frac{1}{2}}$ decay up to an additive term that is linear in the bounded synthesis bias $\varepsilon$.
% \end{corollary}

% \textbf{Remarks.}
% (i) When the learnable blocks synthesize weights with vanishing error ($\varepsilon\!\to\!0$), the bounds reduce to the classical rates.
% (ii) For fixed replacement interval $k$ and stable training, $\varepsilon$ is a small constant determined by how well the neighbor-conditioned synthesis approximates the removed operator; the asymptotic $T^{-\frac{1}{2}}$ behavior is therefore preserved while enjoying lower per-epoch cost.
% (iii) The bounds are agnostic to the CNN/ViT instantiation; only the magnitude of $\varepsilon$
% changes with the specific synthesis rule (Sec.~\ref{sec:cnn_block}-\ref{sec:vit_block}).

% \paragraph{Multi-Replacement error propagation}
% \label{sec:multi_prop}
% Let $\mathcal{F}\subset\{1,\dots,n\}$ be the set of replaced indices and
% assume each full block (including normalization and nonlinearity) is $L$-Lipschitz.
% For $i\in\mathcal{F}$ let $\varepsilon_i$ be the local operator deviation defined in
% Eq.~\eqref{eq:op_dev_def}. Denote by $r:=|\mathcal{F}|$ and
% $\bar\varepsilon := \frac{1}{r}\sum_{i\in\mathcal{F}}\varepsilon_i$,
% $\varepsilon_{\max}:=\max_{i\in\mathcal{F}}\varepsilon_i$.

% \begin{proposition}[Accumulated output deviation]
% \label{prop:acc_dev}
% For any input $\mathbf{x}$,
% \begin{equation}
% \label{eq:bound_approx}
% \begin{aligned}
% &\bigl\|\widehat F(\mathbf{x};\theta,\psi) - F(\mathbf{x};\theta)\bigr\| \\
% &\le
% \begin{cases}
% L^{r}\,\varepsilon_{\max}\,\max\limits_{i\in\mathcal F}\|\mathbf{h}_{i-1}\|,\quad & \text{(worst-case bound)} \\[6pt]
% \dfrac{1-L^{r}}{1-L}\,\bar\varepsilon\,\max\limits_{i\in\mathcal F}\|\mathbf{h}_{i-1}\|,\quad & \text{if } L<1.
% \end{cases}
% \end{aligned}
% \end{equation}
% \end{proposition}

% \begin{proof}
% Insert $\widehat g_i=g_i+(\widehat g_i-g_i)$ at each $i\in\mathcal{F}$ and propagate perturbations.
% For $L<1$, the series of perturbations forms a geometric sum.
% \end{proof}

% \textbf{Implication.}
% When blocks are \emph{non-expansive} ($L\le 1$), e.g., with post-normalization,
% the accumulated discrepancy grows at most linearly with $r$ and is further damped if $L<1$.
% This complements Lemma~\ref{lem:layer_dev_fixed} by accounting for multiple replacements.

% \paragraph{Recoverability and expressivity of the computing layer}
% \label{sec:recoverability}
% We formalize when the learnable block can \emph{exactly} reproduce the removed operator
% ($\varepsilon_i=0$), and what subspace of operators it can represent.

% \noindent\textbf{CNN case.}
% Let the linear part of the removed site be a map $g_i(\mathbf{h})=W_i\mathbf{h}$ (after any fixed alignment used by the baseline).
% The learnable block synthesizes $\widehat W_i=\mathcal{T}_{i-1}(W_{i-1})+\mathcal{T}_{i+1}(W_{i+1})$,
% where $\mathcal{T}_{i\pm1}$ act on the channel modes of their kernel tensors.
% Define the \emph{synthesis span}
% \begin{equation}
%     \mathcal{S}_i \;:=\;
% \Bigl\{\, \mathcal{T}_{i-1}(U)+\mathcal{T}_{i+1}(V)\ :\ U\in\mathcal{U}_{i-1},\ V\in\mathcal{U}_{i+1}\Bigr\},
% \end{equation}
% where $\mathcal{U}_{i\pm1}$ denote the admissible weight tensors with the same shape as $W_{i\pm1}$.

% \begin{lemma}[Exact recoverability in CNNs]
% \label{lem:cnn_recover}
% If $W_i\in\mathcal{S}_i$, then there exist learnable-block parameters such that
% $\widehat W_i=W_i$ and thus $\varepsilon_i=0$.
% \end{lemma}

% \begin{proof}
% By definition of $\mathcal{S}_i$ there exist $U^\star,V^\star$ with
% $W_i=\mathcal{T}_{i-1}(U^\star)+\mathcal{T}_{i+1}(V^\star)$; setting the
% learnable-block weights to realize $(U^\star,V^\star)$ gives the claim.
% \end{proof}

% \noindent\textbf{Rank and span.}
% Write the $1{\times}1$ equivalent of the synthesized operator as a matrix
% $\widehat W_i\in\mathbb{R}^{C^{\text{in}}_{i+1}\times C^{\text{in}}_{i-1}}$.
% Then
% $\mathrm{rank}(\widehat W_i)\le
% \mathrm{rank}\bigl(\mathcal{T}_{i-1}(W_{i-1})\bigr)
% +\mathrm{rank}\bigl(\mathcal{T}_{i+1}(W_{i+1})\bigr)$.
% In typical same-width stages, both terms are full row/column rank, so $\widehat W_i$
% can achieve full rank and does not bottleneck the channel dimension.

% \textbf{To demonstrate its validity, we conduct a brief experimental study.}

% \noindent\textbf{ViT case.}
% In ViT \cite{r14} instantiation, the replacement operator is explicitly constrained to a 2D neighbor span:
% $A_{i}^{\mathrm{RepL}}=\alpha_{i} A_{i-1}+\beta_{i} A_{i+1}$, $\quad M_{i}^{\mathrm{RepL}}=\alpha_{i} M_{i-1}+\beta_{i} M_{i+1}$,
% where $A_{i-1}, A_{i+1} \in \mathbb{R}^{d \times d}\left(\operatorname{resp} . M_{i-1}, M_{i+1}\right)$ are the attention (resp. MLP) operators of the neighboring blocks, and $\alpha_i, \beta_i$ are learned scalars. Thus, by construction, each replaced block is synthesized inside the span of its two neighbors; RepL never introduces an arbitrary new block.

% To quantitatively assess how well the original block is captured by this 2D span, we conduct a feature-space span diagnostic on the same ViT-tiny / CIFAR-10 setting used in our main experiments:

% \textbf{Backbone architecture:} A 12-block ViT-tiny with patch size $8\times 8$, embedding dimension 192, and 3 heads (the same configuration as in our CIFAR-10 experiments).

% \textbf{Training setup:}
% We train a standard backbone ViT (“bp”) with direct backpropagation on CIFAR-10 using the script described in the paper.

% \textbf{Where we probe:} We focus on the block indices that RepL would remove under the same periodic schedule used in the method (remove every 4th block, excluding the last one). In a 12-block ViT-tiny \cite{r14}, this yields the removed indices $i = 2, 6, 10 (0-based)$.

% \textbf{Diagnostic metric:} Let $h_k(x)$ denote the hidden representation after block $k$ for an input $x$. For each removed index $i$, we seek the best approximation
% $h_{i}(x) \approx \tilde{\alpha}_{i} h_{i-1}(x)+\tilde{\beta}_{i} h_{i+1}(x)$, by solving a least-squares problem over CIFAR-10 samples. From this we compute: the relative reconstruction error $r_{i}=\frac{\left\|h_{i}(x)-\Pi_{\mathrm{span}\left(h_{i-1}(x), h_{i+1}(x)\right)}\left(h_{1}(x)\right)\right\|_{2}}{\left\|h_{i}(x)\right\|_{2}}$ aggregated over the dataset. The principal angle (in the 1D case) between $h_i(x)$ and its best neighbor-span reconstruction.

% We use CIFAR-10 \cite{r1} test images, with the same normalization as training, and run the diagnostic on 20 batches (batch size 512). The results for the three removed blocks are:

% \textbf{index $i = 2$: }

% Relative feature-space reconstruction error $r_2 = \mathbf{0.1796}$;

% Principal angle $= \mathbf{7.63^\circ}$; 

% Fitted coefficients $(\tilde{\alpha}_2, \tilde{\beta}_2) \approx (0.4811, 0.5230)$.

% \textbf{index $i = 6$:}

% Relative feature-space reconstruction error $r_6 = \mathbf{0.1501}$; 

% Principal angle $= \mathbf{5.22^\circ}$; 

% Fitted coefficients $(\tilde{\alpha}_6, \tilde{\beta}_6) \approx (0.4711, 0.5325)$.

% \textbf{index i = 10}: 

% Relative feature-space reconstruction error $r_6 = \mathbf{0.1379}$;

% Principal angle $= \mathbf{4.62^\circ}$;

% Fitted coefficients$ (\tilde{\alpha}_{10}, \tilde{\beta}_{10}) \approx (0.4547, 0.5493)$.

% These results show that, measured in terms of their action on real data (hidden representations), the blocks targeted by RepL are well captured by the 2D span of their neighbors: both the relative reconstruction error and the principal angle are small, and the fitted coefficients are close to a symmetric combination of the two neighbors. This empirically supports our modeling choice that a lightweight operator constrained to $\mathrm{span}(A_{i-1}, A_{i+1})$ and $\mathrm{span}(M_{i-1}, M_{i+1})$is sufficient to replace the original block in ViT backbones.

% \begin{lemma}[Exact recoverability in ViTs]
% \label{lem:vit_recover}
% If the linear parts of the removed block satisfy
% $A_i\in\mathrm{span}\{A_{i-1},A_{i+1}\}$ and
% $M_i\in\mathrm{span}\{M_{i-1},M_{i+1}\}$, then
% there exist $(\alpha_i,\beta_i)$ such that $\widehat A_i=A_i$ and $\widehat M_i=M_i$,
% so $\varepsilon_i=0$.
% \end{lemma}

% These statements clarify that $\varepsilon_i$ measures the distance of the removed operator
% to the neighbor-conditioned synthesis span; when that distance is small (as empirically observed),
% the induced bias in Sec.~\ref{sec:error_convergence} remains negligible.

% \paragraph{A simple compute accuracy trade-off for choosing $k$}
% \label{sec:tradeoff_k}
% Let $C_{\mathrm{epoch}}(k)$ denote the per-epoch training cost (FLOPs or wall time)
% under interval $k$, and let $\Delta_{\mathrm{acc}}(k)$ denote the excess risk (or a proxy)
% induced by replacement. From Sec.~\ref{comp} we have the approximation
% $C_{\mathrm{epoch}}(k)\approx \bigl(1-\frac{1}{k}\bigr)C_0$ for a baseline cost $C_0$.
% From Sec.~\ref{sec:error_convergence}, the gradient-norm bound adds an
% $\mathcal{O}(\varepsilon(k))$ bias term. For small replacement rates, we model
% $\varepsilon(k)\approx \frac{c}{k}$ with problem-dependent $c>0$.

% Consider minimizing a weighted objective
% \begin{equation}
% \begin{aligned}
%     J(k) &= \lambda\,C_{\mathrm{epoch}}(k) + \Delta_{\mathrm{acc}}(k), \\[4pt]
%     \Delta_{\mathrm{acc}}(k) &\approx \kappa\,\varepsilon(k) = \frac{\kappa c}{k}.
% \end{aligned}
% \label{eq:cost_def}
% \end{equation}
% where $\lambda,\kappa>0$ encode the user's compute/accuracy preference.
% Using $C_{\mathrm{epoch}}(k)\approx (1-\frac{1}{k})C_0$ gives
% \begin{equation}
%     J(k)\;\approx\; \lambda C_0\Bigl(1-\frac{1}{k}\Bigr) + \frac{\kappa c}{k}
% \;=\; \lambda C_0 \;+\; \frac{\kappa c-\lambda C_0}{k}.
% \end{equation}
% The surrogate suggests a \emph{threshold} behavior: when $\kappa c < \lambda C_0$,
% larger $k$ (more aggressive replacement) is favored; otherwise, a smaller $k$ is preferred.
% In practice, $\kappa c$ can be estimated on a held-out split by measuring the validation loss
% gap as a function of $k$ for a few short runs, after which $k$ is chosen to meet a compute
% budget while keeping the additional bias under the tolerance implied by Corollary~\ref{cor:adam}.
